Complexity of regular abstractions of one-counter languages

We study the computational and descriptional complexity of the following transformation: Given a one-counter automaton (OCA) A, construct a nondeterministic finite automaton (NFA) B that recognizes an abstraction of the language L(A): its (1) downward closure, (2) upward closure, or (3) Parikh image. For the Parikh image over a fixed alphabet and for the upward and downward closures, we find polynomial-time algorithms that compute such an NFA. For the Parikh image with the alphabet as part of the input, we find a quasi-polynomial time algorithm and prove a completeness result: we construct a sequence of OCA that admits a polynomial-time algorithm iff there is one for all OCA. For all three abstractions, it was previously unknown if appropriate NFA of sub-exponential size exist.

==> setfull.tex <==
\newcommand{\onlyappendix}[1]{{\leavevmode\color{blue}#1}}
\newcommand{\onlyappendixpara}[1]{{\textcolor{blue}{#1}}}
\newcommand{\onlymainpaper}[1]{{\leavevmode\color{cyan}#1}}
\newcommand{\onlymainpaperpara}[1]{{\textcolor{cyan}{#1}}}


